Measuring Abuse in Web Push Advertising

The rapid growth of online advertising has fueled the growth of ad-blocking software, such as new ad-blocking and privacy-oriented browsers or browser extensions. In response, both ad publishers and ad networks are constantly trying to pursue new strategies to keep up their revenues. To this end, ad networks have started to leverage the Web Push technology enabled by modern web browsers. As web push notifications (WPNs) are relatively new, their role in ad delivery has not been yet studied in depth. Furthermore, it is unclear to what extent WPN ads are being abused for malvertising (i.e., to deliver malicious ads). In this paper, we aim to fill this gap. Specifically, we propose a system called PushAdMiner that is dedicated to (1) automatically registering for and collecting a large number of web-based push notifications from publisher websites, (2) finding WPN-based ads among these notifications, and (3) discovering malicious WPN-based ad campaigns. Using PushAdMiner, we collected and analyzed 21,541 WPN messages by visiting thousands of different websites. Among these, our system identified 572 WPN ad campaigns, for a total of 5,143 WPN-based ads that were pushed by a variety of ad networks. Furthermore, we found that 51% of all WPN ads we collected are malicious, and that traditional ad-blockers and malicious URL filters are remarkably ineffective against WPN-based malicious ads, leaving a significant abuse vector unchecked.

==> tables/ad_campaign_count.tex <==

\begin{table}[htbp]
\caption{Lists the count of Ad groups and Ads found for identified Ad Campaigns  }

\label{tab:ad_campaigns_count}
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{3cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}}
\toprule
\hline
\multirow{4}*{\textbf{Ad Campaigns}} & \multicolumn{2}{c}{\textbf{Desktop}} & \multicolumn{2}{c}{\textbf{Mobile}} \\
\cline{2-5}
 & \textbf{Ad Groups Count} & \textbf{Ads Count} & \textbf{Ad Groups Count} & \textbf{Ads Count} \\
\hline
 \hline
 Gaming & 2.00\%  & 2.12~\% & 0.66\% & 0.20\%
 \\
 \hline
 Sweepstakes & 10.95\% & 16.41~\% & 7.54\% &3.86\%
 \\
 \hline
 Fake News & 7.40\%& 4.49\% & 10.16\%& 13.16\%
 \\
 \hline
 Fake Alerts &3.24\%  & 6.77\% & 13.77\% & 21.32\%
 \\
 \hline
  Social Media Scam & 1.54\% & 2.2\% & 1.31\% & 0.32\%
 \\
 \hline 
 Fake Alerts(Finance) & 5.70\% & 9.49\% & 4.26\% & 3.82\%
 \\
 \hline
 Scareware & 2.10\% & 8.20\% & 0.66\% & 0.16\%
 \\
 \hline
  Dating & 1.23\% & 0.76\% & 3.60\% & 1.81\%
 \\
 \hline
 Adult Content & 3.24\% & 6.44\% & 24.26\% & 19.5\%
 \\
 \hline
 Health Tips &  5.09\% & 3.86\% & 3.28\% & 1.42\%
 \\
 \hline
  News &  2.31\% & 0.76\% & 3.60\% & 3.94\%
 \\
  \hline
  Other &  55.09\% & 38.48\% & 26.80\% & 30.33\%
 \\
 \hline
 \bottomrule
\end{tabular}}

\end{table}



% \begin{comment}
%  \hline
%  Gaming & 13(2) & 84(20) & 2(1) & 5(2)
%  \\
%  \hline
%  Sweepstakes & 71(34) & 650(445) & 23(6) & 98(27)
%  \\
%  \hline
%  Fake News & 48(30) & 178(103) & 31(15) & 334(237)
%  \\
%  \hline
%  Fake Alerts & 21(12) & 268(192) & 42(13) & 541(320)
%  \\
%  \hline
%   Social Media Scam & 10(2) & 87(33) & 4 & 8
%  \\
%  \hline 
%  Fake Alerts(Finance) & 37(27) & 376(238) & 13(6) & 97(66)
%  \\
%  \hline
%  Scareware & 14(9) & 325(262) & 2(1) & 4(2)
%  \\
%  \hline
%   Dating & 8(2) & 30(5) & 11(6) & 46(21)
%  \\
%  \hline
%  Adult Content & 21(6) & 255(50) & 74 (59) & 495 (437)
%  \\
%  \hline
%  Health Tips &  33(18) & 153(85) & 10 & 36
%  \\
%  \hline
%   News &  15 & 30 & 11 & 100
%  \\
%   \hline
%   Other &  357 & 1524 & 82 & 770
%  \\
%  \hline
%  \hline
%  Total & 648  & 3960 &305  & 2538
%  \\
%  \hline
%  \end{comment}s

==> tables/notifications.tex <==
\begin{figure}[ht]
\caption{Examples of Ad Campaigns }
\begin{center}
\label{text_cluster}
\begin{tabular}{c}
\hline


 \includegraphics[scale=0.28]{figs/notifications.pdf}{C1}

\\
\hline
\hline

 \includegraphics[scale=0.28]{figs/notifications2.pdf}{C2}

 \\
 \hline
    \end{tabular}

\end{center}
\end{figure}


==> tables/suspicious_ads.tex <==

\begin{table}[htbp]
\caption{Measurements on Cluster Groups}
\label{tab:suspicious_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c}

\toprule
\hline

\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}WPN \\ Clusters \\ \end{tabular}}} &  
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Cluster \\ Groups\end{tabular}}} & 
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ad \\ Cluster \\ Groups\end{tabular}}}  & 
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Suspicious \\ Cluster \\ Groups\end{tabular}}}  & 
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Singleton \\ Cluster \\ Groups \end{tabular}}} 

 \\ \hline
 8780 & 2046 & 225 & 325 & 855
 
\\  
\hline
\bottomrule
\end{tabular}}
\end{table}

